The S-PLUS Ultra-Short Survey: first data release

This paper presents the first public data release of the S-PLUS Ultra-Short Survey (USS), a photometric survey with short exposure times, covering approximately 9300 deg$^{2}$ of the Southern sky. The USS utilizes the Javalambre 12-band magnitude system, including narrow and medium-band and broad-band filters targeting prominent stellar spectral features. The primary objective of the USS is to identify bright, extremely metal-poor (EMP; [Fe/H] $\leq -3$) and ultra metal-poor (UMP; [Fe/H] $\leq -4$) stars for further analysis using medium- and high-resolution spectroscopy.}{This paper provides an overview of the survey observations, calibration method, data quality, and data products. Additionally, it presents the selection of EMP and UMP candidates.}{The data from the USS were reduced and calibrated using the same methods as presented in the S-PLUS DR2. An additional step was introduced, accounting for the offset between the observed magnitudes off the USS and the predicted magnitudes from the very low-resolution Gaia XP spectra.}{This first release contains data for 163 observed fields totaling $\sim$324 deg$^{2}$ along the Celestial Equator. The magnitudes obtained from the USS are well-calibrated, showing a difference of $\sim 15$ mmag compared to the predicted magnitudes by the GaiaXPy toolkit. By combining colors and magnitudes, 140 candidates for EMP or UMP have been identified for follow-up studies.}{The S-PLUS USS DR1 is an important milestone in the search for bright metal-poor stars, with magnitudes in the range 10 $ < r \leq 14$. The USS is an ongoing survey; in the near future, it will provide many more bright metal-poor candidate stars for spectroscopic follow-up.

==> table.tex <==

\clearpage
\twocolumn
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{0.3em}

\begin{TableNotes}
\scriptsize
\item[] Notes: 
\item[] The magnitude columns represent values of PStotal and are not corrected for extinction.
\end{TableNotes}

\footnotesize
\onecolumn
\begin{longtable}{>{\footnotesize}c >{\footnotesize}c >{\footnotesize}c >{\footnotesize}c >{\footnotesize}c >{\footnotesize}c >{\footnotesize}c >{\footnotesize}c >{\footnotesize}c >{\footnotesize}c >{\footnotesize}c >{\footnotesize}c >{\footnotesize}c >{\footnotesize}c >{\footnotesize}c}
\caption{Catalog of 140 EMP/UMP candidates} \\
\toprule
 ID             & RA                & DEC     & $r$ & $g$ & $i$ & $z$ & $u$ & $J0378$ & $J0395$ & $J0410$ & $J0430$ & $J0515$ & $J0660$ & $J0861$  \\
(USS) & (Deg) & (Deg) &  &  &  &  &  & & & & & & &             \\ \midrule \midrule
\endfirsthead
%
\multicolumn{15}{c}%
{{\bfseries Table \thetable\ }\textit{(continued)}} \\
\toprule
 ID             & RA                & DEC     & $r$ & $g$ & $i$ & $z$ & $u$ & $J0378$ & $J0395$ & $J0410$ & $J0430$ & $J0515$ & $J0660$ & $J0861$  \\
(USS) & (Deg) & (Deg) &  &  &  &  &  & & & & & & &               \\ \midrule \midrule
\endhead
\hline 
\insertTableNotes  \\
\multicolumn{14}{c}{{Continued on next page}}
\endfoot

\hline 
\insertTableNotes \\
\endlastfoot

SDR1\_SHORTS-STRIPE82\_0004\_0000006 & 1.6576471 & 1.3953081 & 13.12 & 13.59 & 12.89 & 12.81 & 14.55 & 14.20 & 14.18 & 13.92 & 13.80 & 13.44 & 13.05 & 12.87 \\ 
SDR1\_SHORTS-STRIPE82\_0004\_0000108 & 1.1896018 & 1.0214283 & 13.41 & 13.97 & 13.17 & 13.09 & 15.18 & 14.71 & 14.66 & 14.46 & 14.28 & 13.78 & 13.36 & 13.13 \\ 
SDR1\_SHORTS-STRIPE82\_0007\_0000510 & 3.6443336 & -0.71293634 & 13.35 & 13.96 & 13.24 & 12.96 & 14.53 & 14.56 & 14.46 & 14.27 & 14.17 & 13.67 & 13.29 & 13.04 \\ 
SDR1\_SHORTS-STRIPE82\_0008\_0000096 & 4.5058804 & 1.0855886 & 12.94 & 13.62 & 12.67 & 12.52 & 14.95 & 14.44 & 14.43 & 14.15 & 13.98 & 13.40 & 12.91 & 12.56 \\ 
SDR1\_SHORTS-STRIPE82\_0008\_0000210 & 4.401828 & 0.15610152 & 13.92 & 14.56 & 13.67 & 13.55 & 15.89 & 15.54 & 15.16 & 14.97 & 14.92 & 14.33 & 13.83 & 13.61 \\ 
SDR1\_SHORTS-STRIPE82\_0011\_0000366 & 7.6760125 & -1.0947679 & 13.54 & 14.14 & 13.35 & 13.27 & 15.13 & 14.75 & 14.61 & 14.41 & 14.35 & 13.90 & 13.49 & 13.30 \\ 
SDR1\_SHORTS-STRIPE82\_0012\_0000087 & 7.4372125 & 1.1561842 & 12.63 & 13.34 & 12.37 & 12.25 & 15.23 & 14.33 & 14.07 & 14.12 & 13.87 & 13.15 & 12.56 & 12.29 \\ 
SDR1\_SHORTS-STRIPE82\_0014\_0000254 & 7.853146 & 0.20201044 & 13.76 & 14.20 & 13.71 & 13.66 & 15.12 & 14.68 & 14.47 & 14.31 & 14.25 & 13.86 & 13.74 & 13.62 \\ 
SDR1\_SHORTS-STRIPE82\_0018\_0000370 & 10.730438 & 0.23756407 & 12.14 & 12.61 & 11.96 & 11.91 & 13.79 & 13.35 & 13.20 & 12.97 & 12.85 & 12.45 & 12.10 & 11.93 \\ 
SDR1\_SHORTS-STRIPE82\_0018\_0000459 & 11.594033 & 0.44198582 & 13.96 & 14.47 & 13.72 & 13.61 & 15.64 & 15.11 & 15.00 & 14.78 & 14.79 & 14.25 & 13.87 & 13.65 \\ 
SDR1\_SHORTS-STRIPE82\_0018\_0000464 & 10.841239 & 0.4611773 & 14.47 & 14.82 & 14.30 & 14.35 & 15.90 & 15.69 & 15.23 & 15.15 & 15.12 & 14.70 & 14.48 & 14.35 \\ 
SDR1\_SHORTS-STRIPE82\_0020\_0000462 & 13.056526 & 0.35977298 & 12.42 & 13.08 & 12.13 & 12.01 & 14.62 & 14.08 & 13.95 & 13.64 & 13.51 & 12.88 & 12.33 & 12.04 \\ 
SDR1\_SHORTS-STRIPE82\_0021\_0000446 & 14.485071 & -1.0759861 & 14.69 & 15.11 & 14.60 & 14.60 & 16.00 & 15.78 & 15.55 & 15.40 & 15.27 & 14.97 & 14.73 & 14.58 \\ 
SDR1\_SHORTS-STRIPE82\_0023\_0000551 & 16.080364 & -0.78245586 & 14.72 & 15.37 & 14.47 & 14.33 & 16.68 & 16.11 & 16.02 & 15.80 & 15.65 & 15.05 & 14.66 & 14.42 \\ 
SDR1\_SHORTS-STRIPE82\_0025\_0000113 & 16.50135 & -0.30944324 & 14.32 & 14.63 & 14.22 & 14.20 & 15.84 & 15.18 & 14.89 & 14.76 & 14.66 & 14.54 & 14.33 & 14.26 \\ 
SDR1\_SHORTS-STRIPE82\_0028\_0000295 & 19.048897 & 0.7529943 & 14.53 & 14.94 & 14.38 & 14.32 & 15.93 & 15.56 & 15.24 & 15.11 & 15.07 & 14.66 & 14.51 & 14.31 \\ 
SDR1\_SHORTS-STRIPE82\_0031\_0000252 & 20.59981 & -0.6502333 & 13.53 & 14.03 & 13.42 & 13.33 & 14.91 & 14.74 & 14.46 & 14.26 & 14.24 & 13.82 & 13.52 & 13.34 \\ 
SDR1\_SHORTS-STRIPE82\_0033\_0000095 & 21.968967 & -0.27128702 & 14.49 & 14.77 & 14.43 & 14.32 & 15.53 & 15.33 & 14.92 & 14.98 & 14.85 & 14.63 & 14.45 & 14.45 \\ 
SDR1\_SHORTS-STRIPE82\_0034\_0000141 & 22.496855 & 0.10427119 & 13.45 & 14.01 & 13.18 & 13.05 & 15.22 & 14.78 & 14.71 & 14.33 & 14.27 & 13.74 & 13.38 & 13.10 \\ 
SDR1\_SHORTS-STRIPE82\_0034\_0000149 & 22.547462 & 0.14666766 & 10.83 & 11.20 & 10.64 & 10.70 & 12.23 & 11.86 & 11.71 & 11.45 & 11.43 & 11.00 & 10.80 & 10.67 \\ 
SDR1\_SHORTS-STRIPE82\_0050\_0000042 & 34.65409 & 1.3091509 & 14.62 & 15.05 & 14.58 & 14.57 & 15.90 & 15.41 & 15.37 & 15.22 & 15.26 & 14.85 & 14.69 & 14.58 \\ 
SDR1\_SHORTS-STRIPE82\_0050\_0000320 & 33.967308 & 0.735502 & 14.17 & 14.56 & 14.02 & 14.03 & 15.40 & 15.06 & 14.96 & 14.77 & 14.78 & 14.37 & 14.16 & 14.01 \\ 
SDR1\_SHORTS-STRIPE82\_0051\_0000249 & 35.983967 & -1.3795805 & 14.72 & 15.24 & 14.53 & 14.44 & 16.17 & 15.82 & 15.85 & 15.58 & 15.49 & 14.97 & 14.64 & 14.45 \\ 
SDR1\_SHORTS-STRIPE82\_0056\_0000498 & 38.236706 & 0.33034867 & 14.25 & 14.93 & 13.94 & 13.78 & 16.58 & 15.92 & 15.84 & 15.58 & 15.44 & 14.73 & 14.16 & 13.83 \\ 
SDR1\_SHORTS-STRIPE82\_0057\_0000234 & 39.839863 & -1.2754283 & 14.62 & 14.92 & 14.56 & 14.60 & 15.86 & 15.40 & 15.14 & 15.15 & 14.96 & 14.71 & 14.64 & 14.62 \\ 
SDR1\_SHORTS-STRIPE82\_0057\_0000248 & 39.55139 & -1.2515044 & 14.47 & 14.90 & 14.36 & 14.36 & 15.82 & 15.59 & 15.36 & 15.19 & 15.15 & 14.67 & 14.47 & 14.32 \\ 
SDR1\_SHORTS-STRIPE82\_0062\_0000438 & 43.19201 & 0.35812354 & 14.74 & 15.15 & 14.59 & 14.59 & 16.20 & 15.94 & 15.50 & 15.39 & 15.34 & 15.04 & 14.68 & 14.56 \\ 
SDR1\_SHORTS-STRIPE82\_0072\_0000285 & 49.018974 & 0.06775388 & 13.77 & 14.38 & 13.59 & 13.47 & 15.59 & 15.07 & 14.96 & 14.65 & 14.55 & 14.13 & 13.73 & 13.51 \\ 
SDR1\_SHORTS-STRIPE82\_0074\_0000206 & 50.69091 & 0.70975673 & 14.87 & 15.29 & 14.70 & 14.67 & 16.13 & 15.93 & 15.67 & 15.57 & 15.51 & 15.08 & 14.87 & 14.69 \\ 
SDR1\_SHORTS-STRIPE82\_0079\_0000011 & 54.621475 & -0.024894878 & 14.50 & 14.93 & 14.35 & 14.34 & 15.82 & 15.56 & 15.39 & 15.23 & 15.06 & 14.85 & 14.49 & 14.33 \\ 
SDR1\_SHORTS-STRIPE82\_0084\_0000084 & 58.519707 & 1.2353834 & 13.80 & 14.41 & 13.47 & 13.36 & 15.52 & 15.20 & 15.02 & 14.93 & 14.79 & 14.19 & 13.73 & 13.41 \\ 
SDR1\_SHORTS-STRIPE82\_0086\_0000253 & 59.402622 & 0.06786838 & 14.73 & 15.43 & 14.35 & 14.21 & 16.95 & 16.48 & 16.12 & 16.08 & 15.81 & 15.27 & 14.59 & 14.26 \\ 
SDR1\_SHORTS-STRIPE82\_0087\_0000039 & 300.19638 & -0.03680347 & 14.86 & 15.27 & 14.71 & 14.68 & 16.55 & 15.85 & 15.58 & 15.47 & 15.38 & 15.12 & 14.86 & 14.64 \\ 
SDR1\_SHORTS-STRIPE82\_0087\_0000408 & 300.4243 & -0.32248077 & 14.47 & 14.91 & 14.28 & 14.18 & 15.98 & 15.74 & 15.30 & 15.27 & 15.22 & 14.79 & 14.45 & 14.23 \\ 
SDR1\_SHORTS-STRIPE82\_0087\_0001390 & 301.11063 & -0.83181006 & 13.35 & 14.01 & 13.09 & 12.97 & 15.49 & 14.88 & 14.72 & 14.40 & 14.36 & 13.77 & 13.28 & 12.99 \\ 
SDR1\_SHORTS-STRIPE82\_0088\_0000332 & 300.17416 & 1.2281477 & 14.23 & 14.92 & 13.93 & 13.77 & 16.61 & 16.04 & 15.70 & 15.52 & 15.33 & 14.67 & 14.16 & 13.82 \\ 
SDR1\_SHORTS-STRIPE82\_0088\_0000652 & 299.81244 & 1.0351738 & 14.69 & 15.15 & 14.53 & 14.45 & 16.51 & 15.96 & 15.50 & 15.56 & 15.32 & 14.98 & 14.67 & 14.45 \\ 
SDR1\_SHORTS-STRIPE82\_0088\_0001940 & 301.00873 & 0.5642095 & 14.36 & 14.92 & 14.15 & 14.03 & 16.26 & 15.75 & 15.33 & 15.32 & 15.18 & 14.68 & 14.30 & 14.03 \\ 
SDR1\_SHORTS-STRIPE82\_0089\_0000203 & 301.38022 & -0.2050958 & 14.24 & 14.86 & 14.05 & 13.98 & 16.21 & 15.82 & 15.41 & 15.22 & 15.12 & 14.55 & 14.19 & 14.00 \\ 
SDR1\_SHORTS-STRIPE82\_0089\_0000227 & 301.5744 & -0.22473826 & 13.31 & 13.97 & 13.02 & 12.85 & 15.20 & 14.80 & 14.68 & 14.40 & 14.32 & 13.75 & 13.23 & 12.91 \\ 
SDR1\_SHORTS-STRIPE82\_0089\_0000849 & 301.89993 & -1.2271477 & 14.14 & 15.50 & 14.26 & 13.94 & 15.81 & 15.43 & 15.23 & 14.82 & 14.94 & 14.47 & 14.46 & 13.99 \\ 
SDR1\_SHORTS-STRIPE82\_0090\_0000177 & 301.8522 & 1.2722871 & 13.70 & 14.38 & 13.40 & 13.27 & 15.90 & 15.44 & 15.25 & 14.93 & 14.83 & 14.13 & 13.66 & 13.30 \\ 
SDR1\_SHORTS-STRIPE82\_0090\_0000417 & 302.25027 & 1.0935276 & 13.90 & 14.51 & 13.61 & 13.46 & 15.85 & 15.42 & 15.29 & 14.93 & 15.00 & 14.25 & 13.83 & 13.48 \\ 
SDR1\_SHORTS-STRIPE82\_0091\_0000790 & 303.37555 & -0.62275493 & 13.07 & 13.92 & 12.86 & 12.94 & 15.12 & 14.55 & 14.31 & 14.03 & 13.92 & 13.38 & 13.30 & 12.77 \\ 
SDR1\_SHORTS-STRIPE82\_0092\_0000166 & 303.1313 & 1.3386507 & 14.15 & 14.84 & 13.80 & 13.66 & 16.39 & 15.73 & 15.59 & 15.36 & 15.27 & 14.55 & 14.06 & 13.72 \\ 
SDR1\_SHORTS-STRIPE82\_0092\_0000323 & 303.40805 & 1.2786375 & 13.95 & 14.63 & 13.64 & 13.45 & 16.13 & 15.45 & 15.48 & 15.20 & 15.01 & 14.40 & 13.88 & 13.53 \\ 
SDR1\_SHORTS-STRIPE82\_0092\_0002329 & 303.2324 & 0.32604828 & 14.55 & 15.13 & 14.24 & 14.15 & 16.40 & 15.99 & 15.72 & 15.53 & 15.48 & 14.96 & 14.45 & 14.16 \\ 
SDR1\_SHORTS-STRIPE82\_0092\_0003043 & 302.88132 & 0.6380521 & 14.17 & 14.76 & 13.89 & 13.78 & 16.22 & 15.79 & 15.48 & 15.15 & 15.08 & 14.60 & 14.10 & 13.79 \\ 
SDR1\_SHORTS-STRIPE82\_0093\_0000912 & 305.3347 & -1.3431051 & 14.40 & 15.03 & 14.28 & 14.21 & 16.42 & 15.84 & 15.49 & 15.35 & 15.47 & 14.81 & 14.39 & 14.27 \\ 
SDR1\_SHORTS-STRIPE82\_0093\_0001314 & 305.38776 & -0.5404583 & 14.35 & 14.82 & 14.21 & 14.14 & 15.81 & 15.50 & 15.21 & 15.10 & 15.10 & 14.61 & 14.35 & 14.16 \\ 
SDR1\_SHORTS-STRIPE82\_0094\_0000946 & 304.33713 & 0.07345687 & 12.92 & 13.51 & 12.80 & 12.73 & 14.96 & 14.68 & 12.61 & 13.88 & 13.97 & 13.32 & 12.88 & 12.78 \\ 
SDR1\_SHORTS-STRIPE82\_0095\_0000790 & 306.3834 & -1.2881083 & 14.23 & 14.92 & 13.98 & 13.84 & 16.22 & 15.98 & 15.64 & 15.41 & 15.32 & 14.70 & 14.19 & 13.87 \\ 
SDR1\_SHORTS-STRIPE82\_0095\_0001623 & 306.72748 & -0.7906565 & 11.95 & 12.69 & 11.63 & 11.45 & 14.10 & 13.59 & 13.49 & 13.15 & 13.06 & 12.43 & 11.85 & 11.48 \\ 
SDR1\_SHORTS-STRIPE82\_0096\_0000455 & 305.97064 & 1.074333 & 13.61 & 14.37 & 13.25 & 13.08 & 16.02 & 15.38 & 15.28 & 14.96 & 14.74 & 14.16 & 13.50 & 13.11 \\ 
SDR1\_SHORTS-STRIPE82\_0098\_0000172 & 307.9158 & 1.2969278 & 14.65 & 15.26 & 14.45 & 14.34 & 16.45 & 16.26 & 15.75 & 15.56 & 15.62 & 15.07 & 14.62 & 14.34 \\ 
SDR1\_SHORTS-STRIPE82\_0098\_0000565 & 308.04758 & 1.0347829 & 12.77 & 13.33 & 12.56 & 12.46 & 14.43 & 14.01 & 13.94 & 13.69 & 13.59 & 13.10 & 12.71 & 12.46 \\ 
SDR1\_SHORTS-STRIPE82\_0098\_0000877 & 307.21344 & 0.013614895 & 14.54 & 15.14 & 14.28 & 14.19 & 16.53 & 16.17 & 15.74 & 15.44 & 15.47 & 15.04 & 14.45 & 14.22 \\ 
SDR1\_SHORTS-STRIPE82\_0099\_0000111 & 309.29166 & -0.09919771 & 14.64 & 15.05 & 14.53 & 14.52 & 16.19 & 15.93 & 15.41 & 15.40 & 15.20 & 14.85 & 14.64 & 14.55 \\ 
SDR1\_SHORTS-STRIPE82\_0100\_0001569 & 308.3723 & 0.4099422 & 14.23 & 14.80 & 14.05 & 13.91 & 16.01 & 15.69 & 15.36 & 15.16 & 15.16 & 14.62 & 14.21 & 13.94 \\ 
SDR1\_SHORTS-STRIPE82\_0100\_0001740 & 308.47238 & 0.532722 & 14.46 & 14.92 & 14.34 & 14.31 & 16.17 & 15.86 & 13.47 & 15.15 & 15.15 & 14.75 & 14.42 & 14.32 \\ 
SDR1\_SHORTS-STRIPE82\_0101\_0000043 & 310.42578 & -0.048552748 & 14.66 & 15.06 & 14.55 & 14.56 & 16.07 & 15.61 & 15.27 & 15.34 & 15.26 & 14.80 & 14.67 & 14.53 \\ 
SDR1\_SHORTS-STRIPE82\_0101\_0000133 & 311.02887 & -0.15792824 & 13.64 & 14.30 & 13.43 & 13.28 & 15.54 & 15.18 & 15.05 & 14.68 & 14.58 & 13.99 & 13.60 & 13.30 \\ 
SDR1\_SHORTS-STRIPE82\_0101\_0000211 & 310.84012 & -0.24697165 & 14.61 & 14.94 & 14.52 & 14.46 & 15.86 & 15.70 & 15.17 & 15.14 & 15.16 & 14.72 & 14.60 & 14.43 \\ 
SDR1\_SHORTS-STRIPE82\_0101\_0000316 & 310.15854 & -0.37324297 & 14.10 & 14.62 & 13.89 & 13.79 & 15.66 & 15.37 & 15.18 & 14.92 & 14.91 & 14.39 & 14.05 & 13.78 \\ 
SDR1\_SHORTS-STRIPE82\_0101\_0000484 & 310.93823 & -1.3851871 & 14.06 & 14.65 & 14.01 & 13.96 & 15.94 & 15.10 & 15.02 & 14.96 & 14.93 & 14.49 & 14.11 & 13.99 \\ 
SDR1\_SHORTS-STRIPE82\_0101\_0001249 & 310.544 & -0.70014685 & 13.94 & 14.46 & 13.70 & 13.61 & 15.91 & 15.42 & 15.16 & 14.86 & 14.78 & 14.22 & 13.86 & 13.66 \\ 
SDR1\_SHORTS-STRIPE82\_0102\_0000839 & 310.0794 & 0.16043985 & 14.07 & 14.70 & 13.84 & 13.74 & 15.81 & 15.57 & 15.40 & 15.10 & 15.10 & 14.52 & 14.00 & 13.77 \\ 
SDR1\_SHORTS-STRIPE82\_0102\_0000916 & 310.59473 & 0.8105389 & 13.74 & 14.26 & 13.50 & 13.37 & 15.45 & 14.94 & 14.77 & 14.62 & 14.61 & 14.10 & 13.69 & 13.41 \\ 
SDR1\_SHORTS-STRIPE82\_0103\_0000736 & 312.14856 & -1.2355337 & 13.46 & 14.08 & 13.20 & 13.08 & 15.59 & 15.13 & 14.84 & 14.62 & 14.43 & 13.84 & 13.37 & 13.12 \\ 
SDR1\_SHORTS-STRIPE82\_0104\_0000498 & 312.22162 & 0.9273911 & 11.81 & 12.64 & 11.46 & 11.27 & 14.56 & 13.90 & 13.76 & 13.34 & 13.16 & 12.39 & 11.70 & 11.31 \\ 
SDR1\_SHORTS-STRIPE82\_0104\_0001129 & 311.59122 & 0.3266088 & 14.83 & 15.20 & 14.67 & 14.64 & 16.18 & 15.85 & 15.53 & 15.46 & 15.43 & 15.00 & 14.79 & 14.63 \\ 
SDR1\_SHORTS-STRIPE82\_0104\_0001367 & 311.8505 & 0.57589555 & 14.64 & 15.06 & 14.50 & 14.42 & 16.42 & 15.70 & 15.29 & 15.24 & 15.25 & 14.87 & 14.62 & 14.44 \\ 
SDR1\_SHORTS-STRIPE82\_0104\_0001409 & 312.2212 & 0.6251173 & 14.62 & 15.17 & 14.45 & 14.39 & 16.52 & 15.93 & 15.47 & 15.55 & 15.44 & 14.98 & 14.60 & 14.39 \\ 
SDR1\_SHORTS-STRIPE82\_0104\_0001476 & 312.32614 & 0.68522644 & 13.43 & 14.12 & 13.17 & 13.02 & 15.45 & 14.91 & 14.90 & 14.52 & 14.44 & 13.91 & 13.35 & 13.05 \\ 
SDR1\_SHORTS-STRIPE82\_0105\_0000377 & 313.18854 & -0.38996223 & 13.95 & 14.47 & 13.73 & 13.63 & 15.54 & 15.30 & 15.03 & 14.78 & 14.81 & 14.29 & 13.89 & 13.63 \\ 
SDR1\_SHORTS-STRIPE82\_0105\_0000483 & 313.69315 & -0.49006832 & 13.77 & 14.49 & 13.46 & 13.29 & 16.09 & 15.57 & 15.39 & 15.13 & 15.06 & 14.24 & 13.67 & 13.31 \\ 
SDR1\_SHORTS-STRIPE82\_0105\_0000549 & 313.00925 & -1.3846456 & 14.90 & 15.29 & 14.78 & 14.76 & 16.49 & 16.19 & 15.63 & 15.56 & 15.60 & 15.05 & 14.89 & 14.78 \\ 
SDR1\_SHORTS-STRIPE82\_0105\_0000658 & 312.69165 & -1.2699544 & 13.94 & 14.34 & 13.81 & 13.79 & 15.10 & 14.82 & 14.60 & 14.57 & 14.43 & 14.10 & 13.89 & 13.80 \\ 
SDR1\_SHORTS-STRIPE82\_0106\_0000610 & 313.1019 & 0.18768471 & 13.26 & 13.94 & 12.98 & 12.80 & 15.32 & 14.79 & 14.51 & 14.42 & 14.25 & 13.72 & 13.17 & 12.86 \\ 
SDR1\_SHORTS-STRIPE82\_0106\_0000712 & 313.80792 & 0.3431909 & 14.04 & 14.68 & 13.77 & 13.63 & 15.99 & 15.49 & 15.43 & 15.13 & 15.08 & 14.47 & 13.98 & 13.67 \\ 
SDR1\_SHORTS-STRIPE82\_0106\_0000834 & 313.8282 & 0.52028793 & 13.52 & 14.18 & 13.31 & 13.20 & 15.55 & 15.24 & 14.90 & 14.61 & 14.56 & 13.91 & 13.46 & 13.24 \\ 
SDR1\_SHORTS-STRIPE82\_0107\_0000040 & 314.83517 & -0.038442463 & 14.32 & 14.69 & 14.19 & 14.11 & 15.71 & 15.24 & 14.86 & 14.89 & 14.84 & 14.55 & 14.33 & 14.19 \\ 
SDR1\_SHORTS-STRIPE82\_0107\_0000253 & 313.98013 & -0.3653406 & 14.69 & 15.04 & 14.58 & 14.62 & 16.11 & 15.86 & 15.33 & 15.29 & 15.20 & 14.91 & 14.69 & 14.64 \\ 
SDR1\_SHORTS-STRIPE82\_0107\_0000478 & 315.06863 & -1.310828 & 14.44 & 14.87 & 14.30 & 14.26 & 15.92 & 15.48 & 15.13 & 15.02 & 15.00 & 14.63 & 14.43 & 14.32 \\ 
SDR1\_SHORTS-STRIPE82\_0107\_0000942 & 314.30426 & -0.8858297 & 14.42 & 14.80 & 14.26 & 14.20 & 16.16 & 15.50 & 15.13 & 15.08 & 15.03 & 14.63 & 14.38 & 14.23 \\ 
SDR1\_SHORTS-STRIPE82\_0108\_0000333 & 314.37265 & 1.144085 & 14.89 & 15.30 & 14.78 & 14.74 & 16.37 & 16.11 & 15.55 & 15.59 & 15.44 & 15.23 & 14.85 & 14.76 \\ 
SDR1\_SHORTS-STRIPE82\_0108\_0000785 & 314.62006 & 0.07866466 & 12.34 & 13.10 & 12.00 & 11.86 & 14.80 & 14.29 & 14.13 & 13.69 & 13.56 & 12.84 & 12.24 & 11.89 \\ 
SDR1\_SHORTS-STRIPE82\_0108\_0000985 & 314.34805 & 0.7968035 & 14.39 & 14.77 & 14.27 & 14.24 & 15.61 & 15.44 & 15.12 & 15.10 & 14.98 & 14.65 & 14.37 & 14.26 \\ 
SDR1\_SHORTS-STRIPE82\_0108\_0001162 & 314.10263 & 0.2225285 & 12.31 & 14.89 & 14.01 & 13.94 & 13.96 & 13.75 & 13.58 & 13.14 & 15.13 & 14.56 & 14.12 & 12.13 \\ 
SDR1\_SHORTS-STRIPE82\_0108\_0001229 & 314.0349 & 0.27821594 & 14.26 & 14.68 & 14.12 & 14.08 & 15.52 & 15.32 & 15.04 & 15.01 & 14.90 & 14.51 & 14.24 & 14.07 \\ 
SDR1\_SHORTS-STRIPE82\_0109\_0000167 & 316.07025 & -0.13544065 & 14.38 & 15.00 & 14.18 & 14.06 & 16.30 & 16.02 & 15.46 & 15.40 & 15.22 & 14.74 & 14.33 & 14.08 \\ 
SDR1\_SHORTS-STRIPE82\_0109\_0000326 & 315.71826 & -0.28916782 & 14.01 & 14.51 & 13.84 & 13.81 & 15.85 & 15.65 & 12.52 & 14.96 & 14.92 & 14.32 & 13.96 & 13.82 \\ 
SDR1\_SHORTS-STRIPE82\_0109\_0000535 & 316.51276 & -0.50278807 & 14.06 & 14.62 & 13.83 & 13.77 & 15.65 & 15.36 & 15.06 & 14.88 & 14.90 & 14.41 & 13.99 & 13.76 \\ 
SDR1\_SHORTS-STRIPE82\_0109\_0000726 & 315.98138 & -1.2344275 & 13.02 & 13.41 & 12.83 & 12.81 & 14.31 & 13.96 & 13.80 & 13.61 & 13.57 & 13.24 & 12.96 & 12.82 \\ 
SDR1\_SHORTS-STRIPE82\_0109\_0000769 & 316.11676 & -0.8261581 & 13.95 & 14.58 & 13.67 & 13.53 & 15.86 & 15.42 & 15.14 & 14.97 & 14.90 & 14.32 & 13.88 & 13.56 \\ 
SDR1\_SHORTS-STRIPE82\_0109\_0001384 & 316.65747 & -0.77296907 & 14.02 & 14.61 & 13.74 & 13.69 & 15.85 & 15.46 & 15.26 & 14.97 & 14.90 & 14.33 & 13.91 & 13.68 \\ 
SDR1\_SHORTS-STRIPE82\_0109\_0001385 & 315.98273 & -0.7726212 & 13.86 & 14.36 & 13.68 & 14.42 & 15.68 & 15.34 & 15.40 & 15.44 & 14.71 & 14.18 & 14.57 & 14.45 \\ 
SDR1\_SHORTS-STRIPE82\_0109\_0001443 & 315.9575 & -0.71563333 & 13.78 & 14.52 & 13.48 & 13.33 & 16.17 & 15.69 & 15.39 & 15.11 & 14.93 & 14.26 & 13.69 & 13.39 \\ 
SDR1\_SHORTS-STRIPE82\_0113\_0001171 & 319.38544 & -0.9063646 & 13.30 & 14.06 & 12.99 & 12.84 & 15.80 & 15.29 & 15.10 & 14.68 & 14.59 & 13.80 & 13.20 & 12.87 \\ 
SDR1\_SHORTS-STRIPE82\_0115\_0000110 & 320.79617 & -0.10950566 & 14.43 & 14.82 & 14.26 & 14.24 & 16.01 & 15.49 & 15.23 & 15.01 & 14.94 & 14.59 & 14.42 & 14.29 \\ 
SDR1\_SHORTS-STRIPE82\_0116\_0000212 & 320.9774 & 1.0159353 & 14.62 & 14.95 & 14.49 & 14.44 & 15.87 & 15.45 & 15.23 & 15.28 & 15.04 & 14.73 & 14.60 & 14.47 \\ 
SDR1\_SHORTS-STRIPE82\_0116\_0000705 & 320.87167 & 0.46007103 & 14.38 & 14.78 & 14.27 & 14.21 & 15.88 & 15.48 & 15.06 & 15.18 & 14.98 & 14.59 & 14.34 & 14.24 \\ 
SDR1\_SHORTS-STRIPE82\_0116\_0000832 & 320.78775 & 0.700775 & 13.44 & 14.16 & 13.15 & 12.99 & 15.75 & 15.25 & 15.04 & 14.74 & 14.72 & 13.88 & 13.34 & 13.03 \\ 
SDR1\_SHORTS-STRIPE82\_0118\_0000130 & 321.63882 & 1.2726451 & 13.81 & 14.48 & 13.55 & 13.40 & 15.93 & 15.32 & 15.30 & 14.91 & 14.81 & 14.22 & 13.73 & 13.39 \\ 
SDR1\_SHORTS-STRIPE82\_0119\_0000063 & 323.6143 & -0.1691683 & 12.32 & 13.00 & 12.09 & 11.96 & 14.34 & 13.91 & 13.71 & 13.39 & 13.35 & 12.76 & 12.30 & 12.00 \\ 
SDR1\_SHORTS-STRIPE82\_0119\_0000096 & 323.1112 & -0.29941627 & 14.06 & 14.54 & 13.96 & 13.98 & 15.59 & 15.38 & 14.92 & 14.80 & 14.71 & 14.23 & 14.08 & 13.91 \\ 
SDR1\_SHORTS-STRIPE82\_0119\_0000280 & 323.64536 & -1.02573 & 14.24 & 14.66 & 14.20 & 14.17 & 15.52 & 15.11 & 14.79 & 14.72 & 14.80 & 14.48 & 14.26 & 14.22 \\ 
SDR1\_SHORTS-STRIPE82\_0119\_0000315 & 323.36276 & -0.8233687 & 11.94 & 12.77 & 11.81 & 11.68 & 13.91 & 13.66 & 13.40 & 13.28 & 13.11 & 12.43 & 11.81 & 11.65 \\ 
SDR1\_SHORTS-STRIPE82\_0120\_0000668 & 323.40384 & 0.3954084 & 12.03 & 12.35 & 11.93 & 11.90 & 13.17 & 12.86 & 12.61 & 12.54 & 12.44 & 12.20 & 12.00 & 11.93 \\ 
SDR1\_SHORTS-STRIPE82\_0125\_0000766 & 327.80646 & -0.7942097 & 13.78 & 14.35 & 13.51 & 13.38 & 15.49 & 15.09 & 14.93 & 14.78 & 14.65 & 14.13 & 13.70 & 13.43 \\ 
SDR1\_SHORTS-STRIPE82\_0128\_0000568 & 329.0807 & 0.19897743 & 13.55 & 13.95 & 13.44 & 13.41 & 14.80 & 14.51 & 14.29 & 14.13 & 14.12 & 13.81 & 13.54 & 13.41 \\ 
SDR1\_SHORTS-STRIPE82\_0129\_0000049 & 330.816 & -0.0885891 & 14.05 & 14.64 & 13.85 & 13.74 & 15.90 & 15.47 & 15.32 & 15.10 & 14.95 & 14.50 & 14.03 & 13.76 \\ 
SDR1\_SHORTS-STRIPE82\_0131\_0000580 & 331.396 & -0.7343162 & 13.70 & 14.38 & 13.40 & 13.21 & 16.04 & 15.38 & 15.25 & 14.93 & 14.79 & 14.15 & 13.60 & 13.27 \\ 
SDR1\_SHORTS-STRIPE82\_0132\_0000445 & 332.25662 & 0.8650406 & 14.39 & 14.76 & 14.25 & 14.26 & 15.96 & 15.61 & 15.12 & 15.09 & 14.99 & 14.73 & 14.35 & 14.29 \\ 
SDR1\_SHORTS-STRIPE82\_0132\_0000719 & 332.13974 & 0.710427 & 14.40 & 14.88 & 14.22 & 14.19 & 15.91 & 15.75 & 15.39 & 15.28 & 15.28 & 14.79 & 14.35 & 14.22 \\ 
SDR1\_SHORTS-STRIPE82\_0135\_0000179 & 334.06198 & -0.4520497 & 14.08 & 14.60 & 13.86 & 13.81 & 15.94 & 15.38 & 15.22 & 15.19 & 14.88 & 14.41 & 13.99 & 13.82 \\ 
SDR1\_SHORTS-STRIPE82\_0136\_0000079 & 333.86755 & 1.2393587 & 14.91 & 15.32 & 14.86 & 14.79 & 16.11 & 16.07 & 15.56 & 15.45 & 15.43 & 15.21 & 14.93 & 14.85 \\ 
SDR1\_SHORTS-STRIPE82\_0136\_0000384 & 334.59164 & 0.7780391 & 14.31 & 14.98 & 14.00 & 13.85 & 16.71 & 16.08 & 15.75 & 15.60 & 15.36 & 14.81 & 14.21 & 13.87 \\ 
SDR1\_SHORTS-STRIPE82\_0139\_0000295 & 337.55377 & -0.88559717 & 11.66 & 12.44 & 11.31 & 11.15 & 14.25 & 13.59 & 13.48 & 13.12 & 12.95 & 12.22 & 11.57 & 11.20 \\ 
SDR1\_SHORTS-STRIPE82\_0141\_0000013 & 338.9892 & -0.030445319 & 14.66 & 15.06 & 14.57 & 14.51 & 16.28 & 15.60 & 15.31 & 15.25 & 15.27 & 14.84 & 14.65 & 14.48 \\ 
SDR1\_SHORTS-STRIPE82\_0141\_0000105 & 339.17032 & -0.2691278 & 13.21 & 14.04 & 12.83 & 12.67 & 15.97 & 15.44 & 15.19 & 14.91 & 14.58 & 13.75 & 13.09 & 12.70 \\ 
SDR1\_SHORTS-STRIPE82\_0143\_0000035 & 339.82462 & -0.119511425 & 13.91 & 14.55 & 13.66 & 13.53 & 15.81 & 15.43 & 15.28 & 15.14 & 14.95 & 14.26 & 13.85 & 13.54 \\ 
SDR1\_SHORTS-STRIPE82\_0143\_0000283 & 340.15884 & -1.2710394 & 12.22 & 13.06 & 11.86 & 11.69 & 14.96 & 14.33 & 14.17 & 13.75 & 13.59 & 12.80 & 12.11 & 11.74 \\ 
SDR1\_SHORTS-STRIPE82\_0147\_0000322 & 342.71426 & -1.0235988 & 14.70 & 15.07 & 14.53 & 14.48 & 15.96 & 15.79 & 15.49 & 15.31 & 15.25 & 14.92 & 14.68 & 14.50 \\ 
SDR1\_SHORTS-STRIPE82\_0151\_0000121 & 346.32645 & -0.30182838 & 13.98 & 14.37 & 13.84 & 13.86 & 15.58 & 15.15 & 14.79 & 14.70 & 14.56 & 14.24 & 13.95 & 13.84 \\ 
SDR1\_SHORTS-STRIPE82\_0152\_0000423 & 345.2313 & 0.21967787 & 12.38 & 12.80 & 12.20 & 12.23 & 13.74 & 13.40 & 13.27 & 13.08 & 13.02 & 12.68 & 12.32 & 12.18 \\ 
SDR1\_SHORTS-STRIPE82\_0153\_0000034 & 346.71744 & -0.13730732 & 12.64 & 13.21 & 12.46 & 12.42 & 14.28 & 13.91 & 13.71 & 13.51 & 13.51 & 12.93 & 12.59 & 12.43 \\ 
SDR1\_SHORTS-STRIPE82\_0153\_0000307 & 347.2783 & -0.8693464 & 14.01 & 14.33 & 13.82 & 13.80 & 15.58 & 15.15 & 14.70 & 14.67 & 14.62 & 14.16 & 13.94 & 13.88 \\ 
SDR1\_SHORTS-STRIPE82\_0154\_0000195 & 347.83527 & 0.9204981 & 14.14 & 14.58 & 13.90 & 13.86 & 15.89 & 15.53 & 15.20 & 14.98 & 14.85 & 14.43 & 14.06 & 13.86 \\ 
SDR1\_SHORTS-STRIPE82\_0157\_0000444 & 350.66132 & -0.9999145 & 14.18 & 14.52 & 14.07 & 14.04 & 15.44 & 15.06 & 14.83 & 14.77 & 14.68 & 14.40 & 14.18 & 14.06 \\ 
SDR1\_SHORTS-STRIPE82\_0160\_0000250 & 351.24118 & 0.149503 & 14.12 & 14.61 & 13.98 & 14.05 & 15.58 & 15.32 & 15.10 & 15.00 & 14.77 & 14.47 & 14.12 & 14.04 \\ 
SDR1\_SHORTS-STRIPE82\_0160\_0000271 & 351.37036 & 0.5066438 & 13.48 & 14.21 & 13.06 & 12.99 & 16.15 & 15.46 & 15.34 & 14.95 & 14.83 & 14.00 & 13.36 & 13.03 \\ 
SDR1\_SHORTS-STRIPE82\_0161\_0000253 & 353.3934 & -1.3361326 & 12.97 & 13.43 & 12.88 & 12.83 & 14.23 & 13.98 & 13.81 & 13.59 & 13.56 & 13.21 & 12.96 & 12.85 \\ 
SDR1\_SHORTS-STRIPE82\_0161\_0000324 & 353.44833 & -0.5359643 & 14.34 & 14.77 & 14.26 & 14.21 & 15.75 & 15.42 & 15.08 & 14.92 & 14.87 & 14.58 & 14.37 & 14.21 \\ 
SDR1\_SHORTS-STRIPE82\_0161\_0000438 & 353.4584 & -0.9787993 & 14.73 & 15.18 & 14.66 & 14.60 & 16.23 & 15.75 & 15.58 & 15.40 & 15.26 & 15.08 & 14.78 & 14.58 \\ 
SDR1\_SHORTS-STRIPE82\_0162\_0000159 & 353.3701 & 0.9590613 & 14.00 & 14.42 & 13.85 & 13.78 & 15.38 & 15.13 & 14.87 & 14.70 & 14.73 & 14.21 & 13.97 & 13.83 \\ 
SDR1\_SHORTS-STRIPE82\_0163\_0000365 & 353.72775 & -0.95116305 & 12.64 & 13.21 & 12.46 & 12.37 & 14.34 & 13.91 & 13.87 & 13.57 & 13.48 & 12.99 & 12.60 & 12.37 \\ 
SDR1\_SHORTS-STRIPE82\_0166\_0000308 & 355.3462 & 0.28945935 & 13.84 & 14.44 & 13.57 & 13.44 & 15.84 & 15.23 & 15.19 & 15.03 & 14.78 & 14.30 & 13.75 & 13.50 \\ 
SDR1\_SHORTS-STRIPE82\_0166\_0000317 & 355.2404 & 0.34346882 & 13.44 & 13.93 & 13.27 & 13.21 & 15.22 & 14.94 & 13.01 & 14.45 & 14.30 & 13.78 & 13.36 & 13.26 \\ 
SDR1\_SHORTS-STRIPE82\_0169\_0000403 & 358.82654 & -0.8964953 & 13.82 & 14.47 & 13.61 & 13.49 & 15.83 & 15.33 & 15.28 & 14.99 & 14.82 & 14.25 & 13.76 & 13.53 \\ 


\bottomrule

\end{longtable}
\twocolumn
